Graph-Skeleton: ~1% Nodes are Sufficient to Represent Billion-Scale Graph

Due to the ubiquity of graph data on the web, web graph mining has become a hot research spot. Nonetheless, the prevalence of large-scale web graphs in real applications poses significant challenges to storage, computational capacity and graph model design. Despite numerous studies to enhance the scalability of graph models, a noticeable gap remains between academic research and practical web graph mining applications. One major cause is that in most industrial scenarios, only a small part of nodes in a web graph are actually required to be analyzed, where we term these nodes as target nodes, while others as background nodes. In this paper, we argue that properly fetching and condensing the background nodes from massive web graph data might be a more economical shortcut to tackle the obstacles fundamentally. To this end, we make the first attempt to study the problem of massive background nodes compression for target nodes classification. Through extensive experiments, we reveal two critical roles played by the background nodes in target node classification: enhancing structural connectivity between target nodes, and feature correlation with target nodes. Followingthis, we propose a novel Graph-Skeleton1 model, which properly fetches the background nodes, and further condenses the semantic and topological information of background nodes within similar target-background local structures. Extensive experiments on various web graph datasets demonstrate the effectiveness and efficiency of the proposed method. In particular, for MAG240M dataset with 0.24 billion nodes, our generated skeleton graph achieves highly comparable performance while only containing 1.8% nodes of the original graph.

==> 00-table2.tex <==
\begin{table*}[h]
\small
\centering
 \caption{Memory costs for data storage and time costs for graph model training on different datasets.}
 \small
 \resizebox{\textwidth}{!}{
 \begin{tabular}{lcc|lcc|lcc}
  \toprule
  ogbn arxiv & Original & Skeleton-$\gamma$ & Dgraph & Original & Skeleton-$\gamma$ & MAG240M & Original & Skeleton-$\gamma$ \\
  \midrule
  Skeleton Generation & - & 5.2 s & Skeleton Generation & - & 78.5 s & Skeleton Generation & - & ~ 0.5 h \\
  Memory Size & 82 MB & 50 MB & Memory Size & 377 MB & 253 MB & Memory Size & 430 GB & 10 GB\\
  \midrule
  GCN (Epoch 500) & 31.20 s & 22.89 s & GAT (Epoch 200) & 8015.2 s & 4632.6 s & R-SAGE (Epoch 100) & ~ 18.7 h & ~ 9.2 h\\
  SAGE (Epoch 500) & 40.84 s & 30.80 s & SAGE (Epoch 200) & 4280.2 s & 2672.3 s & R-GAT (Epoch 100) & ~ 22.8 h & ~ 15.7 h\\
  \bottomrule
 \end{tabular}
 }
\label{time_all}
\end{table*}
\vspace{-5pt}

==> psedocode/00-code5.tex <==

\begin{algorithm}[h] 
\label{code:conden_c}
    \caption{Condensation-$\gamma$}%算法名字
    \LinesNumbered %要求显示行号
    \KwIn{ Graph $\mathcal{G}=(\mathcal{V},  \mathcal{E})$, target nodes $\mathcal{T}=(T_1,T_2,...,T_n)$, Affiliation and Bridging node set $Affil, Brid$, ego-network's hop $k$}%输入参数
    \KwOut{Condensed graph $\mathcal{G}^\prime=(\mathcal{V}^\prime,  \mathcal{E}^\prime)$}
    Assign each target node $u$ with an unique random 256-bit integer $key[u]$\;
    Set $mask[u]$ to $0$ for every node $u$\;
    \ForEach{target node $u\in \mathcal{T}$}{
        \ForEach{node $v$ in $u$'s $k$-hop ego-network \textbf{with} $v\in Brid$}{
            \tcp{$\odot$ denote Binary Exclusive Or(xor).}
            $mask[v] \gets mask[v] \odot key[u]$\;
        }
    }
    Sort the node by node's $mask$ with Radix Sort\;
    Merge nodes with the same mask into one node\;
    Merge the each affiliation node to its target node and get $\mathcal{G}^\prime$\; 
    \KwRet{$\mathcal{G}^\prime$}
\end{algorithm}
